Principled Bayesian Optimisation in Collaboration with Human Experts

Bayesian optimisation for real-world problems is often performed interactively with human experts, and integrating their domain knowledge is key to accelerate the optimisation process. We consider a setup where experts provide advice on the next query point through binary accept/reject recommendations (labels). Experts' labels are often costly, requiring efficient use of their efforts, and can at the same time be unreliable, requiring careful adjustment of the degree to which any expert is trusted. We introduce the first principled approach that provides two key guarantees. (1) Handover guarantee: similar to a no-regret property, we establish a sublinear bound on the cumulative number of experts' binary labels. Initially, multiple labels per query are needed, but the number of expert labels required asymptotically converges to zero, saving both expert effort and computation time. (2) No-harm guarantee with data-driven trust level adjustment: our adaptive trust level ensures that the convergence rate will not be worse than the one without using advice, even if the advice from experts is adversarial. Unlike existing methods that employ a user-defined function that hand-tunes the trust level adjustment, our approach enables data-driven adjustments. Real-world applications empirically demonstrate that our method not only outperforms existing baselines, but also maintains robustness despite varying labelling accuracy, in tasks of battery design with human experts.

==> figs/human_AI_collab_frame.tex <==
\usetikzlibrary{graphs, quotes}
\tikz{  
  \node (boa) [rectangle, draw] at (-4.2,0) {BO algorithm};
  \node (hl) [rectangle, draw] at (1,0) {Label Agent};
  \node (bf) [rectangle, draw] at (7.2,0) {Black-box Function};

\coordinate (A) at (-4.2,2);
\coordinate (B) at (7.2,2);

 \draw[-] (boa) -- (A);
  \draw[-] (A) -- (B) node[midway, above]{Adjustable direct query}; 

\graph [nodes={circle,draw}, 
          ] 
{ (boa) ->[transform canvas={yshift=0.1cm}, "Propose $x_t$"] (hl);
  (hl) ->[transform canvas={yshift=-0.1cm}, "If `bad', reject $x_t$"] (boa);
  (hl) -> ["If `good', evaluate at $x_t$"] (bf);
 (bf) ->[bend left, very thick, dotted, "\texttt{Scalar evaluation feedback}"] (boa);
  
 (B) ->[ ] (bf);
};
  \draw[bend right, very thick, dotted,->] (hl) to node [yshift=1.5ex] {\texttt{\quad Agent classification feedback}} (boa);

%
%(bf) ->[bend left, very thick, dotted, "Scalar evaluation feedback"] (boa); 

}
% \usetikzlibrary {graphs}
% \tikz \graph {
%   "$x_1$" -> "$x_2$"[red] -> "$x_3,x_4$";
%   "$x_1$" ->[bend left] "$x_3,x_4$";
% };
